Graph Matching via convex relaxation to the simplex

This paper addresses the Graph Matching problem, which consists of finding the best possible alignment between two input graphs, and has many applications in computer vision, network deanonymization and protein alignment. A common approach to tackle this problem is through convex relaxations of the NP-hard \emph{Quadratic Assignment Problem} (QAP). Here, we introduce a new convex relaxation onto the unit simplex and develop an efficient mirror descent scheme with closed-form iterations for solving this problem. Under the correlated Gaussian Wigner model, we show that the simplex relaxation admits a unique solution with high probability. In the noiseless case, this is shown to imply exact recovery of the ground truth permutation. Additionally, we establish a novel sufficiency condition for the input matrix in standard greedy rounding methods, which is less restrictive than the commonly used `diagonal dominance' condition. We use this condition to show exact one-step recovery of the ground truth (holding almost surely) via the mirror descent scheme, in the noiseless setting. We also use this condition to obtain significantly improved conditions for the GRAMPA algorithm [Fan et al. 2019] in the noiseless setting.

==> preamble.tex <==
\usepackage[margin=1in]{geometry}
 
%\usepackage[]{amsmath,amssymb,epsfig}
% \usepackage{subfigure}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb,epsfig}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{comment}
\usepackage{array}
\usepackage{algorithm}
\usepackage{url}
\usepackage{enumitem}   
\usepackage{lscape}
\usepackage{algpseudocode}
\usepackage{setspace}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{color}
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{esvect}
\usepackage{diagbox}
\usepackage{bbm}
%\usepackage{slashbox}
% \usepackage{hyperref}
\usepackage{bm}
\usepackage{enumitem}  
\usepackage[pagewise]{lineno}\linenumbers
\usepackage{placeins}
\usepackage{hyperref}
\usepackage[%
    font={small,sf},
    labelfont=bf,
    format=hang,    
    format=plain,
    margin=0pt,
    width=0.8\textwidth,
]{caption}
\usepackage[list=true]{subcaption}

%amsart
%\usepackage[affil-it]{authblk}
\usepackage{amsaddr}

%-----------------------------
% Theorem like environments
%-----------------------------
\newtheorem{theorem}{Theorem}
% \theoremstyle{plain}
\newtheorem{acknowledgment}{Acknowledgment}
\newtheorem{assumption}{Assumption}
\newtheorem{axiom}{Axiom}
\newtheorem{case}{Case}
\newtheorem{claim}{Claim}
\newtheorem{conclusion}{Conclusion}
\newtheorem{condition}{Condition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{criterion}{Criterion}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{exercise}{Exercise}
\newtheorem{lemma}{Lemma}
\newtheorem{notation}{Notation}
\newtheorem{problem}{Problem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{solution}{Solution}
\newtheorem{summary}{Summary}
\numberwithin{equation}{section}
\newtheorem{thmx}{Theorem}
\renewcommand{\thethmx}{\Alph{thmx}}
%\newtheorem{proof}{Proof}
\makeatletter
\def\paragraph{\@startsection{paragraph}{4}%
  \z@\z@{-\fontdimen2\font}%
  {\normalfont\bfseries}}
\makeatother

\newenvironment{rcases}
  {\left.\begin{aligned}}
  {\end{aligned}\right\rbrace}
	
	\renewcommand{\thefootnote}{\arabic{footnote}} 
	
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\ddiag}{ddiag}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\maximize}{maximize}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\spn}{span}
%---------------------------------------------
% Commands for symbols used in the report.
% \mathcal symbols
%----------------------------------------------
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calPp}{\ensuremath{\calP^{\prime}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}

%estimator
\newcommand{\est}[1]{\widehat{#1}}
\newcommand{\hatx}{\est{X}}
\newcommand{\hatxp}{\est{X}_{\calP}}

% Miscellaneous symbols 
\newcommand{\tri}{\ensuremath{\bigtriangleup}}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\ceil}[1]{\left\lceil{#1}\right\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\dotprod}[2]{\langle#1,#2\rangle}
%\newcommand{\est}[1]{\hat{#1}}
\newcommand{\expec}{\ensuremath{\mathbb{E}}}
\newcommand{\matR}{\ensuremath{\mathbb{R}}}
\newcommand{\matN}{\ensuremath{\mathbb{N}}}
\newcommand{\matZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
\newcommand{\Linfnorm}{L_{\infty}}
\newcommand{\todo}[1]{\textbf{TODO: #1}}
\newcommand{\logit}{\operatorname{logit}}
% 
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\newcommand{\hemant}[1]{\textcolor{blue}{HT: #1}}
\newcommand{\ea}[1]{\textcolor{brown}{EA: #1}}
\newcommand{\alternative}[1]{\textcolor{applegreen}{#1}}

%Indicator variable
\newcommand{\ones}{\ensuremath{\mathbf{1}}} 

% Vectors and matrices
\newcommand{\vecx}{\mathbf x}
\newcommand{\vecn}{\mathbf n}
\newcommand{\vecp}{\mathbf p}
\newcommand{\vecq}{\mathbf q}
\newcommand{\veci}{\mathbf i}
\newcommand{\vecj}{\mathbf j}
\newcommand{\vecu}{\mathbf u}
\newcommand{\vecv}{\mathbf v}
\newcommand{\vecw}{\mathbf w}
\newcommand{\vecb}{\mathbf b}
\newcommand{\vecm}{\mathbf m}
\newcommand{\vecc}{\mathbf c}
\newcommand{\vecy}{\mathbf y}
\newcommand{\vecf}{\mathbf f}
\newcommand{\vecz}{\mathbf z}
\newcommand{\veca}{\mathbf a}
\newcommand{\vecg}{\mathbf g}
\newcommand{\veco}{\mathbf 0}
\newcommand{\matA}{\ensuremath{\mathbf{A}}}
\newcommand{\matB}{\ensuremath{\mathbf{B}}}
\newcommand{\matI}{\ensuremath{\mathbf{I}}}
\newcommand{\matV}{\ensuremath{\mathbf{V}}}
\newcommand{\matH}{\ensuremath{\mathbf{H}}}
\newcommand{\matX}{\ensuremath{\mathbf{X}}}
\newcommand{\matP}{\ensuremath{\mathbf{P}}}


% Paper specific commands

\newcommand{\tauset}[1]{{#1{\tau}}_{\pi^*,K}}
\newcommand{\tautil}{\tauset{\tilde}}
\newcommand{\taucheck}{\tauset{\check}}
\newcommand{\taupi}{\tauset{}}
\newcommand{\taupisph}{\taupi\cap\mathbb{S}^{{n^2}-1}}
\newcommand{\taupiball}{\taupi\cap\mathbb{B}^{{n^2}-1}}
%comands of a previous paper (take what can be useful)
\newcommand{\lip}{\ensuremath{M}}
\newcommand{\complincmat}{\ensuremath{C}} 
\newcommand{\normvecglob}[1]{\frac{#1}{\abs{#1}}}
\newcommand{\normvec}[1]{\frac{#1}{\norm{#1}_2}}
\newcommand{\Dinv}{D_{w^*}^{-1}}
\newcommand{\Dw}{D_{w^*}}
\newcommand{\westr}{\est{w}^r}
\newcommand{\zestr}{\est{z}^r}
\newcommand{\wstarr}{w^{*,r}}
\newcommand{\zstarr}{z^{*,r}}
\newcommand{\Lv}{L_V(\lambda)}
\newcommand{\Ldag}{L^\dagger(\lambda)}
\newcommand{\Lvdag}{L_V^\dagger(\lambda)}
\newcommand{\Ltildev}{L_{\tilde V}(\lambda)}
\newcommand{\Ltildevdag}{L_{\tilde V}^\dagger(\lambda)}
\newcommand{\Lcom}{L_{\operatorname{com}}}
\newcommand{\bmax}{b_{\max}}
\newcommand{\Cnt}{C_{n,T,\delta}}
\newcommand{\Clt}{C_{L,T}}
\newcommand{\inv}[1]{{#1}^{-1}}
\newcommand{\Vtildeinv}{\tilde V^{-1}}
\newcommand{\ymin}{y^*_{\min}}
\newcommand{\yminL}{y^{*^L}_{\min}}
\newcommand{\Emax}{\calE_{\max}}
\newcommand{\Emin}{\calE_{\min}}
\newcommand{\Perm}{\calP_n}
\newcommand{\Birk}{\calB_n}
%\newcommand{\ones}{\mathbbm{1}}
\newcommand{\lamin}{\lambda_{\operatorname{min}}}
\newcommand{\lamax}{\lambda_{\operatorname{max}}}
\newcommand{\okap}{\overline{\kappa}}

\newcommand{\lfreqsp}{\calV_{\tau}}
\newcommand{\hfreqsp}{\calV^{\perp}_{\tau}}
\newcommand{\lfreqproj}{P_{\calV_{\tau}}}
\newcommand{\hfreqproj}{P_{\calV^{\perp}_{\tau}}}
\newcommand{\simp}[1]{\bm{\mathit{\Delta}}_{#1}}

\def\id{\operatorname{Id}}
\def\Xzero{X^{(0)}}
\def\Xone{X^{(1)}}
\def\Xk{X^{(k)}}
\def\Xkone{X^{(k+1)}}
\def\Xkon{X^{(k-1)}}
\def\Yone{X^{(1)}}
\def\Xl{X^{(l)}}
\def\greedy{\texttt{GMWM}}
\def\tsuper{{(t)}}
\def\tsuperone{{(t+1)}}
\def\superzero{{(0)}}
\def\vec{\operatorname{vec}}
\def\simpn2{\bm{\mathit{\Delta}}_{n^2}}
\def\popgradient{\overline{\nabla E}}
\def\gradE{\nabla E}
\def\oN{\overline{N}}
\def\er{Erd\H{o}s-R\'enyi }
\def\piopt{\pi^{\operatorname{opt}}}
\def\Xopt{X^{\operatorname{opt}}}
\def\Piopt{\Pi^{\operatorname{opt}}}
%\def\hadexp{\stackrel{\odot}{\exp}}
\def\hadexp{\exp_{\odot}}
\def\mdgm{\texttt{EMDGM}}
\def\pgdgm{\texttt{PGDGM}}
\def\LEinf{L_{E,\infty}}
\def\LE2{L_{E,2}}
\def\grampa{\texttt{Grampa}}
\def\qpadmm{\texttt{QPADMM}}
\def\blAtilde{\bm{\tilde{A}}}
\def\vtil{{\tilde{v}}^{(1)}}
\def\vtilT{{\tilde{v}}^{(1)T}}
\def\vtilk{{\tilde{v}}^{(1,2)}}
\def\vtilkT{{\tilde{v}}^{(1,2)T}}
\def\Xgrampa{\hat{X}_{\operatorname{grampa}}}
\def\leta{\Lambda_\eta}
\def\ileta{\Lambda^{(-1)}_\eta}
\def\blambda{\bm{\lambda}}
\def\diag{\operatorname{diag}}
\def\gmsimp{{\calG\calM}_{\operatorname{simplex}}}
\def\gmsimpless{{\calG\calM}^{\operatorname{noiseless}}_{\operatorname{simplex}}}
\def\gmK{{\calG\calM}_{\calK}}
\def\prop{\operatorname{suff.cond.}}
\def\propsym{\operatorname{suff.cond.}_{sym}}

\newcommand{\rev}[1]{\textcolor{red}{#1}}

==> previous_material/PGD.tex <==
%%gradient descent 
\subsection{Gradient descent dynamics}
\label{sec:dynamics}
We propose to solve the convex relaxations of graph matching of the form \eqref{eq:QAP_convex_obj} by using a projected gradient descent algorithm. Our analysis will be focus on the theoretical guarantees of this method, knowing that for constraint convex problems with unique global solution (for example when the problem is strongly convex), the gradient descent iterates are guaranteed to converge to the global minimizer. The gradient descent dynamics possesses two steps, as described below, 

\begin{enumerate}
    \item \textbf{Steepest descent update.} At each step we move our current optimizer candidate in the direction given by the gradient of $E(X)$ evaluated at that candidate \[Y^{(t+1)}=X^{(t)}-\gamma_t (A^2X^{(t)}+X^{(t)}B^2-2AX^{(t)}B),\] 
    where $\gamma_t>0$ are a sequence of parameters, usually referred to as the learning rates. Let us rewrite this step in vector notation, recalling the lower case convention described in Sec.\ref{sec:notation}. 
    \begin{equation}
        y^\tsuperone =(\id\otimes\id-\gamma_t H ) x^\tsuper, 
    \end{equation}
    where $H=(\id\otimes A-B\otimes \id)^2$.
    \item \textbf{Projection step. } To update the optimizer candidate, we project $Y^{(t)}$ onto the set of constraints $\calK$, that is, 
    \[X^{(t+1)}=\tau_{\calK}(Y^{(t+1)}),\]
    where $\tau_{\calK}(\cdot)$ is the $\elle_2$ projection operator onto $\calK$. Note that, given the convexity of $\calK$, there is a unique solution to the projection problem. 
\end{enumerate}
Often, we will write more compactly 
\begin{equation}\label{eq:dynamic_compact}
    X^\tsuperone= \tau_\calK\circ\calL_H(X^\tsuper,\gamma_t),
\end{equation}
where $\calL_H(X,\gamma_t)=X-\gamma_t(A^2X+XB^2-2AXB)$ for a matrix $X$, or equivalently in vector notation $\calL_H(x,\gamma_t)=(\id-\gamma_tH)x$. In general, the function $\tau_K\circ \calL_H$ is nonlinear, which in inherited from the nonlinearity of the projection operator, which we described further in the next section. 


\ea{Some points of discussion on 10/02 about the G.D dynamics: 
\begin{itemize}
    \item See how statistical guarantees of G.D has been obtained in the literature. For example, Yuxin Chen for the regularized MLE in the ranking problem (leave-one technique, etc)/
    \item Very roughly, an idea of what we want to prove would be as follows. We would like that at some point $k'\in \matN$, $X^{(k')}$ enters into the Voronoi cell of $X^*=\id$ and stay there for all $k>k'$. One difficulty is that the limit $\lim_{k\to \infty}X^\tsuper$ is hard to characterize (via KKT for example) except in the case $\calH$(even there is hard to know if one can go much further with the elements given in \cite{Grampa}).
    \item One possible way to achieve that goal is to consider the property defined in \eqref{eq:property} as a metric or proxy defining how close where are to the Voronoi. We know that if all pairs $(i,j)$ satisfy this property, then we are in the Voronoi. The challenge is to prove that there exists a point in time $k''\in \matN$ such that for all $k>k''$ there is a strict monotonicity (except if already attained its maximum) in the number of pairs satisfying \eqref{eq:property}. Since, the number of pairs satisfying this property is a natural number, the fact that is strictly mononotical implies that converge to it maximum. 
    \item Another related strategy is to analyse the trajectories of the process in the noiseless case, prove that in that case the process hit the right Voronoi cell and stay there, first. Then find a good norm (maybe $\ell_\infty$), and prove that the trajectories of the noisy case are not that far from the ones in the noiseless case(recalling that the limit point of the process changes with the addition of noise, but the ground truth is assumed fixed, then also the Voronoi cell is fixed). 
\end{itemize}
}


\ea{An idea that can helps to simplify the analysis of the projection operator is to use the \emph{softplus} function, defined as $\operatorname{softplus}(x)=\log(1+e^{\kappa x})/\kappa$ for some parameter $\kappa>1$ that controls the degree of approximation. This function is strictly monotone, which implies that, when applied entrywise, it left the property \eqref{eq:property} invariant.} 


%%projections onto convex sets
\subsection{Projections onto $\calK$}
Let us consider the problem of projecting a matrix in $\matR^{n\times n}$ onto the different possibilities for the (convex) constraint set $\calK$. We consider the possibilities $\calK\in \{\triangle_{n}, \calH, \check{\calB}\}$, where $\calH$ is the set of matrices $X\in \matR^{n\times n}$ that satisfy $\ones^TX\ones=n$, $\triangle_n$ is the set of matrices that belong to the intersection of $\calH$ and the cone of matrices with non-negative entries, which is the $n$-simplex on $\matR^{n^2}$. On the other hand, $\check{\calB}$ represents the set of right stochastic matrices, defined by $\check{\calB}=\{X\in \matR^{n\times n}: X\geq 0,\enskip X\ones=\ones\}$. 

The following lemma helps to characterize the operator $\tau_{\calK}$.
\begin{lemma}\label{lem:projection}
    Let $Y\in \matR^{n\times n}$, then \begin{enumerate}[label=(\roman*)]
        \item $\tau_{\calH}(Y)=Y-\nu J$, where $\nu=\frac1{n^2}(\ones^TY\ones-n)$.
        \item $\tau_{\triangle}(Y)=(Y-\nu J)_+$, for some $\nu\in \matR$. Here $(\cdot)_+$ represents the function $x\rightarrow \max\{0,x\}$ applied entrywise. The value of $\nu$ can be founded by solving the following \[\langle J, (Y-\nu J)_+\rangle_F=n,\]
        for which there exist efficient algorithms. See \cite{Condat} for a fast method and references on the subject. Given that in this case, projecting onto $\check{\calB}$ corresponds to project each row onto a unit simplex, the same methods described in \cite{Condat}, to find the values of $\nu_i$, apply. In particular, given the separability of the problem, it can be efficiently parallelized. 
        \item $\tau_{\check{\calB}}(Y)_{i:}=(Y_{i:}-\nu_i\ones^T)_+$, for some real values $\{\nu_i\}^n_{i=1}$. Here, for a matrix $M$, we define $M_{i:}$ as its $i$-th row. 
    \end{enumerate}
\end{lemma}

\ea{summary about discussion on friday 10/02 about the projection: 
\begin{itemize}
    \item Clearly $\tau_\calH$ is linear (global shift) in terms of $Y$, so it is easier to understand. This should be equivalent to grampa dynamics without the regularization. 
    \item There is a region $\calR_0$ on $\matR^{n\times n}$, with $\operatorname{Leb}(\calR_0)\neq 0$, where the two projections $\tau_\calH$ and $\tau_\triangle$ coincide. I believe we can characterize this region as $\calR_0=\{X\in \matR^{n\times n}: X=M+\eta J,\enskip M\in \triangle\}$, using the fact that $J$ is the "normal vector" to $\calH$(maybe it's easier to visualize in the vector form). 
    \item It may be possible to partition the set of matrices $\matR^{n\times n}$ into different sets, one of them being $\calR_0$, where we have a "good idea" of the action of $\tau_\triangle$. This looks non trivial, but it will ultimately depends on the precision that is needed. The main takeaway is that altough this is a non-linear function, it might be have a "lower complexity" in regions and hopefully (finger crossed) our gradient descent process avoid the high complexity parts. This remains to be seing. 
    \item TODO: search in the literature some analysis of projections onto $\triangle$ or $\check{B}$, maybe even in the fully deterministic setting. 
\end{itemize}
}

%%further look into the dynamics
\subsection{Unwrapping the dynamics}\label{sec:unwrap}
In general, it is hard to unwrap the gradient descent dynamic \eqref{eq:dynamic_compact}, given its inherent nonlinearity. However, in some cases we can obtain a clean expression for the iterates. 

We start with the hyperplane case $\calK=\calH$. In addition, we will make the simplifying assumption that $\gamma_t$ is a constant $\gamma$. In this case, it is easy to see that 
\begin{equation}
    x^\tsuper=(\id-\gamma H)^tx^\superzero-\sum^t_{j=1}\nu_{j-1}(\id-\gamma H)^{t-j}\ones,
\end{equation}
where \[\nu_{j-1}=\nu\big((\id-\gamma H)x^{(j-1)}\big)=\frac1{n^2}\Big(\langle (\id-\gamma H)x^{(j-1)},\ones\rangle-n\Big).\] By our choice of initial point $x^\superzero=\frac{\ones}n$, we can write
\begin{equation}
    x^\tsuper=-\sum^t_{j=0}\nu_{j-1}(\id-\gamma H)^{t-j}\ones,
\end{equation}
where we define $\nu_{-1}:=\frac{-1}n$. We can write more explicitly the sequence $\nu_t$. Indeed, notice that we can obtain a recursion for $\nu$ as follows,
\begin{align*}
    \nu_t&=\frac1{n^2}(\langle (\id-\gamma H)x^{(t-1)},\ones\rangle -n)\\
    &=\frac1{n^2}\big(\langle -\sum^t_{j=0}\nu_{j-1}(\id-\gamma H)^{t-j+1}\ones,\ones\rangle-n\big).
\end{align*}
As an example, we have $\nu_0=\frac{-\gamma}{n^2}\langle H\ones,\ones\rangle$, $\nu_1=-\nu_0+\frac1{n^2}\langle(\frac{\gamma^2 H^2}n+(\gamma\nu_0-2\frac{\gamma}{n})H)\ones,\ones\rangle$.
As a first step in the analysis, we study the dynamics when replacing $H$ by its expected value. It is worth noting that by doing that, the dynamic \eqref{eq:dynamic_compact} became deterministic. The following lemma gives us the expected value of $H$. 
\begin{lemma}
We have 
\begin{equation}
    \expec(H) = (2+\sigma^2)\big(\frac{n+1}n\big)\id \otimes \id -\frac2n\big(\vec(\id)\vec(\id)^T+T\big),
\end{equation}
where $T\in \matR^{n^2\times n^2}$ is the matrix representing the transpose transpose transformation in $\matR^{n\times n}$.
\end{lemma}
\begin{proof}
A simple calculation shows that 
\begin{align*}
    \expec(H)&=\expec(\id\otimes A^2)+\expec(B^2\otimes \id)-2\expec(B\otimes A)\\
    &=\expec(\id\otimes A^2)+\expec(A^2\otimes \id)+\sigma^2\expec(Z^2\otimes \id)-2\expec(A\otimes A).
\end{align*}
From this and Lemma \ref{lem:expec_GOE_sq}, the conclusion follows.
\end{proof}


==> previous_material/analysis.tex <==
%%%analysis
\section{Analysis}\label{sec:analysis}
%
%previous proof of thm3 with some imprecisions
 % Defining the events 
    % %
    % \begin{equation*}
    %     \calE' = \left\{X\neq \frac1n\id\right\}, \enskip
    %     \calE'' = \left\{X = \sum^n_{i=1}\mu_iv_iv^T_i\text{ and }X\in \simpn2\right\}, \enskip
    %     \calE  = \calE'\cap\calE'',
    % \end{equation*}
    % %
    % our objective is to control the probability of $\calE$. Consider the following partition of $\calE'=\calE'_1\cup\calE'_2\cup\calE'_3$, where 
    % %
    % \begin{equation*}
    %     \calE'_1 = \{X\in \calI\}, \enskip
    %     \calE'_2 = \{X\in\calR_1\}\cap \calE', \enskip
    %     \calE'_3  = \{X\in \calR_2\}\cap \calE',
    % \end{equation*}
    % %
    % where $\calR_1$ corresponds to the class of reducible matrices with a Frobenius normal form having at least one block of size one, and similarly, $\calR_2$ denotes the class of reducible matrices with a Frobenius normal form with all of its blocks of size two or more. Notice that $\{X\in \calI\}$ is strictly contained in $\calE'$. To bound the probability of $\calE$, we will bound separately the probability of the events $\calE'
    % _1\cap \calE''$, $\calE'_2\cap\calE''$ and $\calE'_3\cap\calE''$. 
    % %
    % \paragraph{Bounding $\prob(\calE'
    % _1\cap \calE'')$.} Notice that for an $X\in \calE''\cap\calE'_1$, the strong form of the Perron-Frobenius theorem applies, given that $X$ is irreducible, and its entries are nonnegative. This implies, in particular, that there exists $i'\in[n]$ such that either $v_{i'}(k)>0$ for all $k\in [n]$, or $v_{i'}(k)<0$ for all $k\in [n]$ (here $v_{i'}(k)$ denotes the $k$-th coordinate of $v_{i'}$). Then clearly
    % %
    % \begin{equation*}
    %     \calE'_1\cap\calE''\subseteq\{\exists i' \text{ s.t. } v_{i'}(k)>0,\forall k\in[n]\}\cup \{\exists i' \text{ s.t. } v_{i'}(k)<0,\forall k\in[n]\}.
    % \end{equation*}
    % %
    % We will need the following lemma, whose proof can be found in Appendix \ref{app:proof_prob_unif_sphere}. 
    % %
    % \begin{lemma}\label{lem:proba_pos_eigenvectors}
    % Let $v_1,v_2,\ldots,v_n$ be a set of (not necessarily independent) vectors uniformly distributed on the unit sphere $\mathbb{S}^{n-1}$. Then it holds
    % %
    % \begin{equation*}
    %     \prob(\exists i'\in[n]  \text{ s.t. } v_{i'}(k)>0,\forall k\in[n])\leq \frac{n}{2^n}.
    % \end{equation*}
    % %
    % \end{lemma}
    % %
    % Using Lemma \ref{lem:proba_pos_eigenvectors}, we conclude that 
    % %
    % \begin{equation}\label{eq:boundproba1}
    %     \prob(\calE'_1\cap\calE'')\leq \frac{n}{2^{n-1}}. 
    % \end{equation}
    % %
    \paragraph{Bounding $\prob(\calE'
     _2\cap \calE'')$.} 
     %Recall that
    % %
    % \begin{equation*}
    %     X\in \calR \iff \exists m< n \text{ and } P\in\calP_n\text{ s.t }PXP^T=\operatorname{blockdiag}(B_{11},\ldots,B_{mm})\text{ with }B_{kk}\in \matR^{n_k\times n_k}.
    % \end{equation*}
    % %

        
    %%%%%%%%
    %%%%%%%%
 %    Given that for $X\in \calE'_2$ there is at least one block of size one, we can assume w.l.o.g. that $B_{11}\in \matR$. Moreover, if $X\in \calE'_2\cap\calE''$ we have $B_{11}\geq 0$, because the fact $X$ has positive coordinates implies that the same it is true for all blocks $B_{kk}$ in its Frobenius normal form. On the event $\calE'_1\cap\calE''$ we have, denoting $e_1$ the first element of the canonical basis of $\matR^n$
 %    %
 %    \begin{align}
 %         PXP^Te_1&=B_{11}e_1\nonumber\\
 %         \implies XP^Te_1 &= B_{11}P^Te_1\nonumber\\
 %         \implies\sum^n_{i=1}\mu_iv_i\langle v_i,P^Te_1\rangle &= B_{11}P^Te_1\nonumber\\ \label{eq:mu_D}
 %         \implies VD\bm{\mu}&=B_{11}P^Te_1,
 %    \end{align}
 %    %
 % where $V$ has as columns the eigenvectors $v_1,\ldots, v_n$, $D$ is a diagonal matrix with entries $D_{ii}=\langle v_i,P^Te_1\rangle$ and $\bm{\mu}=(\mu_1,\ldots,\mu_n)^T$. We have the following simple result. 
 % %
 % \begin{claim}\label{claim:D_invert}
 %     D is a.s. invertible 
 % \end{claim}
 % %
 %    \begin{proof}
 %        $D$ is invertible iff $D_{ii}\neq 0$ for all $i\in [n]$. Note that, there exists $k'\in[n]$ (the image of $1$ under the permutation map associated to $P^T$), such that 
 %        \begin{equation*}
 %            \forall i\in[n], \enskip \langle v_i,P^Te_1\rangle = v_i(k').
 %        \end{equation*}
 %        On the other hand, given that $v_i$ is uniformly distributed on $\mathbb{S}^{n-1}$, it is clear that for any $k\in[n]$ $\prob(v_i(k)=0)=0$. 
 %    \end{proof}
 %    %
    % Claim \ref{claim:D_invert} implies that $VD$ is a.s. invertible, which in turn implies that there exists $\bm{\mu}$ that satisfies $VD\bm{\mu}=B_{11}P^Te_1$. On the other hand, it is clear that $\bm{\mu}=B_{11}\ones$ is a solution, which is associated with $X=B_{11}\id$. Given that on the event $\calE''$, $X\in \simpn2$, then $B_{11}$ has to be $\frac1n$, but on the event $\calE'_2$ we have $X\neq \frac1n\id$. This leaves no choice other than $\prob(\calE'_2\cap\calE'')=0$.
    % %
    %
    Consider the following block decomposition of $\tilde{A}$
    %
    \begin{equation*}
        \tilde{A}=\begin{bmatrix}
            \blAtilde_{11}& \blAtilde_{12}&\cdots&\blAtilde_{1m}\\
            \blAtilde_{21}& \blAtilde_{22}&\ddots&
            \vdots\\
            \vdots& & \ddots & \\
            \blAtilde_{m1}&\cdots & &\blAtilde_{mm},
        \end{bmatrix}
    \end{equation*}
    %
    where $\blAtilde_{kl}$ belongs to $\matR^{n_k\times n_l}$ (we use bold notation here to distinguish $\blAtilde_{kl}$ from the $(k,l)$ entry of $\tilde{A}$). Observe that $\blAtilde_{kl}=\blAtilde_{lk}^T$. With this, it is easy to verify that
    %
    \begin{equation*}
        \tilde{A}PXP^T = PXP^T\tilde{A} \iff \blAtilde_{kl}B_{ll}=B_{kk}\blAtilde_{kl}, \enskip \forall k,l\in [m],
    \end{equation*}
    %
    which implies that 
    %
    \begin{equation}\label{eq:block_commuting1}
        \blAtilde_{lk}\blAtilde_{kl}B_{ll}=B_{ll}\blAtilde_{lk}\blAtilde_{kl},\enskip \forall k,l \in[m] \text{ with }k\neq l,
    \end{equation}
    %
    and 
    %
    \begin{equation}\label{eq:block_commuting2}
        \blAtilde_{ll}B_{ll}=B_{ll}\blAtilde_{ll},\enskip \forall l \in[m].
    \end{equation}
    %
    
    
    %%%%%%%%%
    %%%%%%%%%%%
    \paragraph{Bounding $\prob(\calE'
    _3\cap \calE'')$.} On the event $\calE'
    _3\cap \calE''$, we have $PXP^T=\operatorname{blockdiag}(B_{11},\ldots,B_{mm})$, with all the blocks $B_{kk}\in \matR^{n_k\times n_k}$ having size $n_k\geq 2$. We note that 
    %
    \begin{equation*}
        AX=XA\iff \tilde{A}PXP^T = PXP^T\tilde{A},
    \end{equation*}
    %
    where $\tilde{A}:=PAP^T$. Consider the following block decomposition of $\tilde{A}$
    %
    \begin{equation*}
        \tilde{A}=\begin{bmatrix}
            \blAtilde_{11}& \blAtilde_{12}&\cdots&\blAtilde_{1m}\\
            \blAtilde_{21}& \blAtilde_{22}&\ddots&
            \vdots\\
            \vdots& & \ddots & \\
            \blAtilde_{m1}&\cdots & &\blAtilde_{mm},
        \end{bmatrix}
    \end{equation*}
    %
    where $\blAtilde_{kl}$ belongs to $\matR^{n_k\times n_l}$ (we use bold notation here to distinguish $\blAtilde_{kl}$ from the $(k,l)$ entry of $\tilde{A}$). Observe that $\blAtilde_{kl}=\blAtilde_{lk}^T$. With this, it is easy to verify that
    %
    \begin{equation*}
        \tilde{A}PXP^T = PXP^T\tilde{A} \iff \blAtilde_{kl}B_{ll}=B_{kk}\blAtilde_{kl}, \enskip \forall k,l\in [m],
    \end{equation*}
    %
    which implies that 
    %
    \begin{equation}\label{eq:block_commuting1}
        \blAtilde_{lk}\blAtilde_{kl}B_{ll}=B_{ll}\blAtilde_{lk}\blAtilde_{kl},\enskip \forall k,l \in[m] \text{ with }k\neq l,
    \end{equation}
    %
    and 
    %
    \begin{equation}\label{eq:block_commuting2}
        \blAtilde_{ll}B_{ll}=B_{ll}\blAtilde_{ll},\enskip \forall l \in[m].
    \end{equation}
    %
    It can be seen that the following facts hold. 
    %
    \begin{enumerate}[label=(\roman*)]
        %
        \item $\tilde{A}\stackrel{dist.}{=}A\sim GOE(n)$. In particular, $B_{ll}\sim GOE(n_l)$. Recal$\blAtilde_{l'l'}$ has $n_{l'}$ different eigenvalues almost surely (see \cite[Thm. 2.5.2]{anderson_guionnet_zeitouni_2009})
        %
        \item $\blAtilde_{lk}\blAtilde_{kl}=\blAtilde_{lk}\blAtilde_{lk}^T\sim Wish(n_l,n_k)$ for all $k\neq l\in [m]$. Here $M\sim Wish(n_1,n_2)$ means that $M\in \matR^{n_1\times n_1}$ can be written $M=\tilde{M}\tilde{M}^T$, where $\tilde{M}\in \matR^{n_1\times n_2}$ is a matrix with independent standard Gaussian entries. This corresponds to the classic Wishart distribution. 
        %
        \item $\blAtilde_{lk}\blAtilde_{kl}$ is independent from $\blAtilde_{ll}$, for all $l\neq k$.
    \end{enumerate}
    %
From \eqref{eq:block_commuting1} and \eqref{eq:block_commuting2}, we deduce that 
%
\begin{align*}
    \calE'_3\cap\calE''&\subseteq \{\forall l\in[m]: B_{ll}\text{ satisfies }\eqref{eq:block_commuting1} \text{ for all }k\neq l, \text{ and }\eqref{eq:block_commuting2}\}\\
    &\subseteq \{B_{l'l'}\text{ satisfies }\eqref{eq:block_commuting1} \text{ for all }k\neq l', \text{ and }\eqref{eq:block_commuting2}\}\\
    &\subseteq \{B_{l'l'}\text{ satisfies }\eqref{eq:block_commuting1} \text{ for }k'\neq l', \text{ and }\eqref{eq:block_commuting2}\},
\end{align*}
%
where $k',l'\in[m]$ are any pair satisfying
%
\begin{align*}
    l'&\in \arg \min \limits_{j\in[m]}n_j\\
    k'&\in \arg \min \limits_{j\in[m]\setminus{l'}}n_j.
\end{align*}
%
It is a well-known fact of the Wishart distribution, given the definitions of $k',l'$, that $\blAtilde_{l'k'}\blAtilde_{k'l'}$ has $n_{l'}$ different eigenvalues with probability $1$ (it can be seen as a consequence of \cite[Prop. 4.1.3]{anderson_guionnet_zeitouni_2009}). Similarly, $\blAtilde_{l'l'}$ has $n_{l'}$ different eigenvalues almost surely (see \cite[Thm. 2.5.2]{anderson_guionnet_zeitouni_2009}). This implies that the eigenvectors of $\vtil_1,\ldots,\vtil_{n_{l'}}$ are uniquely defined up to a global sign change, and the same it is true for $\vtilk_1,\ldots,\vtilk_{n_{l'}}$. From this, we deduce that 
%
\begin{equation*}
    \calE'_3\cap\calE''
    \subseteq \{B_{l'l'}=\sum^{n_{l'}}_{i=1} b^{(l')}_i\vtil_i \vtilT_i\}\cap\{B_{l'l'}=\sum^{n_{l'}}_{i=1} b^{(l',k')}_i\vtilk_i \vtilkT_i\}\cap \{B_{l'l'}\in \calI\}, 
\end{equation*}
%
where for all $i\in[n_{l'}]$, $b^{(l')}_i$ and $b^{(l',k')}_i$ are real numbers. By virtue of the Perron-Frobenius theorem (which applies because $B_{l'l'}\in\calI$ and has nonnegative entries) we have that
\begin{align*}
    \calE'_3\cap\calE''&\subseteq \{\exists i',i''\in[n_{l'}]\text{ s.t. }b^{(l')}_{i'},b^{(l',k')}_{i''} \text{ have multiplicity one}\}\\
    &\subseteq \{\exists i',i''\in[n_{l'}]\text{ s.t. }\vtil_{i'}=\vtilk_{i''}\text{ or }\vtil_{i'}=-\vtilk_{i''}\}.
\end{align*}
Remark that, by the fact $(i)$ above, the vectors $\{\vtil_i\}^{n_{l'}}_{i=1}$ form a basis and are marginally uniformly distributed on $\mathbb{S}^{n-1}$. Similarly, by the fact $(ii)$, $\{\vtilk_i\}^{n_{l'}}_{i=1}$ are marginally uniformly distributed on $\mathbb{S}^{n-1}$. 
By the fact $(iii)$, for any pair $i',i''\in[n_{l'}]$, $\vtil_{i'}$ and $\vtilk_{i''}$ are independent. From this, we deduce that $\prob(\vtil_{i'}=\vtilk_{i''})=\prob(\vtil_{i'}=-\vtilk_{i''})=0$, for any $i',i''\in[n_{l'}]$. Hence, $\prob(\calE'_3\cap\calE'')=0$.

==> previous_material/main_results_prev.tex <==
%%main results
\section{Main results}\label{sec:main_results}

As a first step in the analysis, we give a result for the first iteration of the projected gradient descent dynamic when the initialization is given by $X^{(0)}=J/n$. We start with the analysis of the noiseless case $\sigma=0$, that is, when $B=A$ (recall that we assumed w.l.o.g that $\Pi^*=\id$).

\begin{proposition}[First iteration in the noiseless case]
Let $X^{(0)}=J/n$ and $Y^{(1)}=X^{(0)}-\gamma(A^2X^{(0)}+X^{(0)}A^2-2AX^{(0)}A)$, for a $\gamma>0$. Then $Y^{(1)}$ is symmetric and satisfies \eqref{eq:property_sym} almost surely. In addition, it holds that $\Xone_{\calH}:=\tau_{\calH}(\Yone)$ is symmetric and satisfies \eqref{eq:property_sym} a.s, thus $\greedy(\Xone_\calH)=\id$ a.s. 
\ea{We need an statement about the other projections.}
\end{proposition}
\begin{proof}
The fact that $Y^{(1)}$ is symmetric follows directly from the fact that $X^{(0)}$ and $A$ are symmetric. To prove the rest, we divide $Y^{(1)}$ in three terms, the first is $\Xzero$, the second is $-\gamma(A^2\Xzero+\Xzero A^2)$ and the third is $\gamma A\Xzero A$. It is clear from its definition that $\Xzero$ that it satisfies \[\Xzero_{ii}+\Xzero_{jj}=2\Xzero_{ij},\]
for all $i\neq j\in[n]$. Take $i\neq j\in [n]$, and define $a_k$ as the $k$-th column of $A$, then for the second term we have, \begin{align*}
(A^2\Xzero+\Xzero A^2)_{ij}&=\langle a_i,\sum^n_{k=1}a_k\Xzero_{kj}\rangle+\langle \sum^n_{k=1}a_k\Xzero_{ik}, a_j\rangle\\
&=\langle \frac1n\sum^n_{k=1}a_k,a_i+a_j\rangle,
\end{align*} 
which clearly implies that $M:=(A^2\Xzero+\Xzero A^2)$ satisfies $M_{ii}+M_{jj}=2M_{ij}$. For the third term, define $M'=A\Xzero A$. We have that $M'=\frac1n AJA$, then clearly \begin{equation*}
    M'_{ii}+M'_{jj}-2M'_{ij}=\frac1n\langle (a_i-a_j), J(a_i-a_j)\rangle, 
\end{equation*}
from the fact that $J$ is psd we have that  $M'_{ii}+M'_{jj}-2M'_{ij}\geq 0$. To prove that the previous quantity is strictly positive, it is sufficient to prove that $\langle a_i-a_j, \ones\rangle \neq 0$ (given the null space of $J$ is $\operatorname{span}^\perp\{\ones\}$). Define $g_{ij}=(a_i-a_l)/\sqrt{2}$, which is distributed as mean zero Gaussian vector with covariance $\Sigma_{ij}$. A simple calculation yields, 
\begin{equation*}
    \Sigma_{ij}=\frac1n \id- \frac1{2n}(e_ie_j^T+e_je_i^T),
\end{equation*}
where $\{e_k\}^n_{k=1}$ are the elements of the canonical basis of $\matR^n$. Since the matrix $\Sigma_{ij}$ is positive definite, we can define $\Sigma^{\frac12}_{ij}$ and $\Sigma^{-\frac12}_{ij}$. With this, we have 
\begin{equation*}
    \langle g_{ij},\ones\rangle=\langle\Sigma^{\frac12}_{ij}\Sigma^{-\frac12}_{ij}g_{ij},\ones \rangle=\langle \tilde{g}_{ij},\Sigma^{\frac12}_{ij}\ones \rangle,
\end{equation*}
where $\tilde{g}_{ij}\sim \calN(0,\id/n)$. From this, given that $\Sigma^{\frac12}_{ij}\ones$ is a fixed vector, it is easy to see that the event $\langle \tilde{g}_{ij},\ones \rangle=0$ has probability zero. From Lemma \ref{lem:projection} part $(i)$, we see that $\Xone_\calH=\tau_\calH(\Yone)$ is symmetric because $\Yone$ is symmetric. Using the fact that property \eqref{eq:property_sym} is closed under global translation (given in Lemma \ref{lem:property_preserving_ops}) we deduce that $\Xone$ satisfy \eqref{eq:property_sym}. 
\end{proof}

%%%%%proposition 2
\begin{proposition}\label{prop:pop_dyn_multistep}
    Assume that $\{\Xk\}^\infty_{k=0}$ is a trajectory of the dynamic defined by \eqref{eq:pop_dyn_init} and \eqref{eq:pop_dyn_update} with step size sequence $\{\gamma_k\}^\infty_{k=0}\in \matR^\matN_+$. In addition, if $\sigma\neq 0$ we assume that $\sum^\infty_{l=0}\gamma_l<\frac{2\gamma_0n}{(n+1)\sigma^2}$. Then $\greedy(\Xk)=\id$ for all $k\in \matN$. 
\end{proposition}

%proof of prop
\begin{proof}[Proof of Proposition \ref{prop:pop_dyn_multistep}]
    We will prove that $\Xk$ satisfy the diagonal dominance property. For that, using \eqref{eq:Xkone_Xk}, \eqref{eq:lemma_gradmat3} and Lemma \ref{lem:Xk_pop_dyn}    \begin{equation*}
        \frac{\Xk_{11}}{\Xk_{12}}= \frac{\Xzero_{11}}{\Xzero_{12}}\exp{\big(\sum^{k-1}_{l=0}\gamma_l(a_\sigma X^{(l)}_{12}-(a_\sigma-2) X^{(l)}_{11})\big)},
    \end{equation*}
    where $a_\sigma:=2+\frac{n+1}n\sigma^2$. We deduce that 
    \begin{equation*}
        \frac{\Xk_{11}}{\Xk_{12}}= \exp{\big(\frac{2\gamma_0}n+\sum^{k-1}_{l=0}\gamma_l(a_\sigma X^{(l)}_{12}-(a_\sigma -2)X^{(l)}_{11})\big)}.
    \end{equation*}
    From Lemma \ref{lem:Xk_pop_dyn}, we know that the diagonal elements are all equal, which imposes the bound $X^{(l)}_{11}\leq 1$ for all $l$. On the other hand, $X^{(l)}_{12}\geq 0$ for all $l$. All this implies that   \begin{equation*}
        \frac{\Xk_{11}}{\Xk_{12}}\geq \exp{\big(\frac{2\gamma_0}n-(a_\sigma -2)\sum^{k-1}_{l=0}\gamma_l\big)}.
    \end{equation*}
    In the case $\sigma=0$, we have that $a_\sigma-2=0$, so for any step size sequence with $\gamma_0>0$ we have that $\Xk_{11}>\Xk_{12}$. If $\sigma\neq 0$ and the step size sequence is such that $\sum^\infty_{l=0}\gamma_l<\frac{2\gamma_0n}{(n+1)\sigma^2}$ then clearly $\Xk_{11}>\Xk_{12}$, which by Lemma \ref{lem:Xk_pop_dyn}, gives that $\Xk_{ii}>\Xk_{ij}$ for all $i\neq j$. We conclude that $\greedy(\Xk)=\id$. 
\end{proof}
\ea{I feel this is too pesimistic and wasteful...see Proposition below...}

==> previous_material/nonused_material.tex <==
We take $u\in \matR^n\setminus{0}$ such that $\ones^Tu=0$, and compute 
    \begin{align*}
        -u^T\popgradient (\Xk)u&=-(2+\sigma^2)(\frac{n+1}n)u^T\Xk u+\frac2n\Tr(\Xk)u^Tu+\frac2nu^T\Xk u\\
        &=-(2+\sigma^2\frac{n+1}n)u^T\Xk u+\frac2n\Tr(\Xk)u^Tu\\
        &=-(2+\sigma^2\frac{n+1}n)(\Xk_{11}\sum^n_{i=1}u^2_i+\Xk_{12}\sum_{i\neq j}u_iu_j)+2\Xk_{11}\sum^n_{i=1}u^2_i\\
        &=-(2+\sigma^2\frac{n+1}n)\Xk_{12}\sum_{i\neq j}u_iu_j-\sigma^2\frac{n+1}n\Xk_{11}\sum^n_{i=1}u^2_i.
    \end{align*}
   But given that $\sum_{i,j}u_iu_j=0=\sum^n_{i=1}u^2_i+\sum_{i\neq j}u_iu_j$, we deduce that 
   \[
-u^T\popgradient (\Xk)u=\Big((2+\sigma^2\frac{n+1}n)\Xk_{12}-\sigma^2\frac{n+1}n\Xk_{11}\Big)\sum^n_{i=1}u^2_i
   \]
   Using that $n\Xk_{11}+n(n-1)\Xk_{12}=n$, and recalling the definition $a_\sigma:=2+\frac{n+1}n\sigma^2$, we get 
   \[
-u^T\popgradient (\Xk)u=\big((2+\sigma^2(n+1))\Xk_{12}-\sigma^2\frac{n+1}n\big)\|u\|^2
   \]
   
   %$\sum_{i\neq j}u_iu_j<0$, hence $u^T\popgradient (\Xk)u>0$.
   \subsection{Some experiments regarding concentration for $\nabla E$}
\ea{This is probably just for our understansing...We should choose a few figures to display at the end.}

\paragraph{Noiseless case.} We simulate $A\sim GOE(n)$ and plot the histogram of certain entries of $\nabla E(\Xzero)$ and $\nabla E(\Xone)$. In Fig. \ref{fig-grad_0_a} and \ref{fig-grad_0_b} we plot the histogram of a pair of entries of $\nabla E(J/n)$(entries $(1,1)$ and $(1,2)$). The idea is to have a feel of how a typical diagonal element and an off-diagonal element look like. We use $n=500$ and $100$ Monte Carlo runs to generate this plot. In Fig. \ref{fig-grad_0_c} we plot the entries of $\nabla E(J/n)$, also for $n=500$, but in only one realization. The principle is to understand how the entries of the terms in our updates look like. 

\begin{figure}[h!]
  \begin{subfigure}[t]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/histogram_grad11_0.jpg}
    \caption{Entry $(1,1)$ of $\nabla E(J/n)$ for $100$ Monte Carlo.}
    \label{fig-grad_0_a}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/histogram_grad12_0.jpg}
    \caption{Entry $(1,2)$ of $\nabla E(J/n)$ for $100$ Monte Carlo.}
    \label{fig-grad_0_b}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/histogram_grad_0.jpg}
    \caption{Entries of $\nabla E(J/n)$ one realization.}
    \label{fig-grad_0_c}
  \end{subfigure}
  \caption{Histogram for the distribution of the entries of $\nabla E(J/n)$ for $n=500$.} 
  \label{fig:histo_grad_0}
\end{figure}

\begin{figure}[ht]
  \begin{subfigure}[t]{0.43\textwidth}
    \includegraphics[width=\textwidth]{images/diag_grad_0.jpg}
    \caption{Diagonal entries of $\nabla E(J/n)$ one realization.}
    \label{fig-grad_0_a_dia}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.43\textwidth}
    \includegraphics[width=\textwidth]{images/off_grad_0.jpg}
    \caption{Off-diagonal entries of $\nabla E(J/n)$ one realization.}
    \label{fig-grad_0_b_off}
  \end{subfigure}
  \caption{Histogram for the distribution of diagonal and off-diagonal entries $\nabla E(J/n)$ for $n=500$.} 
  \label{fig:histo_grad_0_diagoff}
\end{figure}

\begin{figure}[h!]
  \begin{subfigure}[t]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/histogram_grad11_1.jpg}
    \caption{Entry $(1,1)$ of $\nabla E(\Xone)$ for $100$ Monte Carlo.}
    \label{fig-grad_1_a}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/histogram_grad12_1.jpg}
    \caption{Entry $(1,2)$ of $\nabla E(\Xone)$ for $100$ Monte Carlo.}
    \label{fig-grad_1_b}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.33\textwidth}
    \includegraphics[width=\textwidth]{images/histogram_grad_1.jpg}
    \caption{Entries of $\nabla E(\Xone)$ one realization.}
    \label{fig-grad_1_c}
  \end{subfigure}
  \caption{Histogram for the distribution of the entries of $\nabla E(\Xone)$ for $n=500$.} 
  \label{fig:histo_grad_1}
\end{figure}

\begin{figure}[ht]
  \begin{subfigure}[t]{0.43\textwidth}
    \includegraphics[width=\textwidth]{images/diag_grad_1.jpg}
    \caption{Diagonal entries of $\nabla E(\Xone)$ one realization.}
    \label{fig-grad_1_a_dia}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.43\textwidth}
    \includegraphics[width=\textwidth]{images/off_grad_1.jpg}
    \caption{Off-diagonal entries of $\nabla E(\Xone)$ one realization.}
    \label{fig-grad_1_b_off}
  \end{subfigure}
  \caption{Histogram for the distribution of diagonal and off-diagonal entries $\nabla E(\Xone)$ for $n=500$.} 
  \label{fig:histo_grad_1_diagoff}
\end{figure}

\todo{See what happens with more iterations. Put the statistics regarding the diag.dominance v/s sufficient property. }

\subsection{Noiseless case}
We first consider the case $\sigma=0$, in which case we have $A=B$. In this case, we proved that every iterate of the gradient descent dynamic is symmetric, when the initial point is $J/n$. Therefore, by Lemma \ref{lem:sufficient_prop} we know that \eqref{eq:property_sym} implies \eqref{eq:property} in this case. 

To motivate the study of property \eqref{eq:property} and, in the case of symmetry, of property \eqref{eq:property}, we track the evolution of the three quantities defined below, in the gradient descent dynamic. More precisely, at each iteration $t\in \matN$ we compute:
\begin{itemize}
    \item $q^{(t)}= \frac{|(i,j)\in[n]^2:(i,j)\text{ satisfies \eqref{eq:property_sym} for} X^\tsuper|}{n(n-1)}$, which is the fraction of pairs that satisfy \eqref{eq:property_sym}.
    \item $r^{(t)}=\frac{|i\in [n]: X^\tsuper_{ii}>X^\tsuper_{ij}\text{for all }j\neq i|}{n}$, that is the fraction of rows with diagonal dominance property.
    \item $s^{(t)}=\frac{\langle X^{(t)}_{\calP},\id\rangle_F}n$, where we define $X^{(t)}_{\calP}:=\texttt{GMWM}(X^{(t)})$. This quantity represents the overlap of $X^{(t)}_{\calP}$ with the ground truth (assumed to be $X^*=\id$). 
\end{itemize}

\begin{figure}
    \centering
\includegraphics[scale=0.3]{images/simplex_traject_1_mean.jpg}
    \caption{Evolution of the quantities $q^{(t)},r^\tsuper,s^\tsuper$ for the average of $10$ Montecarlo trajectories of projected (onto $\triangle$) gradient descent.}
    \label{fig:qrs_evol}
\end{figure}
In Figure \ref{fig:qrs_evol}, we plot the values of $q^\tsuper,r^\tsuper,s^\tsuper$ for $t=1,2,\cdots,30$ when considering projected gradient descent for the problem with simplex constraints, that is, $\calK=\triangle$. Here, the matrix $A$ is of size $n=500$. This figure suggests that $q^\tsuper$ is better correlated with $s^\tsuper$ than $r^\tsuper$. We see a similar phenomenon in the case of $\texttt{Grampa}$ algorithm, as can be seen in Table \ref{tab:qrs_grampa} (in particular see the column for $\sigma=0$). In the case of Grampa algorithm, we used the exact characterization of the solution $X_{\operatorname{grampa}}$, given in spectral form. For that reason, the quantities $q,r,s$ are defined using $X_{\operatorname{grampa}}$ instead of $X^\tsuper$, in the obvious way. 

\subsection{Case $\sigma\neq 0$}

\begin{table}[h!]
    \centering
    \begin{tabular}{c||c|c|c|c}
       \diagbox{}{$\sigma$} & 0 & 0.05 & 0.1 & 0.3\\
        \hline
        q &  1 & 1 & 1& 0.997\\
        r & 0.625 & 0.613 & 0.566&   0.255\\
        s & 1 & 1 & 1 & 0.556
    \end{tabular}
    \caption{Comparison between the quantities $q,r,s$ for Grampa algorithm with $n=1000$, averaged over $10$ Montecarlo runs.}
    \label{tab:qrs_grampa}
\end{table}


\begin{lemma}\label{lem:sequence_gap_popdyn}
For any sequence $\{g_k\}^\infty_{k=1}>1$ for which it holds 
\begin{equation*}
    \frac{\sigma^2(n+1)}{\sigma^2(n+1)+2n}g_k<1,
\end{equation*}
there exist a sequence $\{\gamma_k\}^\infty_{k=0}\in\matR_+$ such that the iterates $\Xk$(in $\matR^{n\times n}$) of the dynamic defined by \eqref{eq:pop_dyn_init} and \eqref{eq:pop_dyn_update} satisfies the following
\begin{equation}\label{eq:ratio_1211}
\frac{\Xk_{12}}{\Xk_{11}}= \frac{\sigma^2(n+1)}{\sigma^2(n+1)+2n}g_k,
\end{equation}
for all $k\geq 1$.
\end{lemma}
\begin{proof}
We will use induction. Recall that, by definition,
\begin{align*}
    \Xkone_{11}&=\overline{N}^{-1}_k \Xk_{11}\exp{(-\gamma_k(a_\sigma-2)\Xk_{11})}\\
     \Xkone_{12}&=\overline{N}^{-1}_k \Xk_{12}\exp{(-\gamma_ka_\sigma\Xk_{12})}.
\end{align*}
For the base case $k=1$, we have that \[\frac{\Xone_{12}}{\Xone_{11}}=e^{-2\gamma_0/n^2},\]
hence we can choose $\gamma_0=\frac{n^2}{2}\log{\frac{\sigma^2(n+1)+2n}{\sigma^2(n+1)g_1}}$. Now we prove that if \eqref{eq:ratio_1211} is true for $k$, then it also holds for $k+1$. We have 
\begin{align*}
  \frac{\Xkone_{12}}{\Xkone_{11}}  &=\frac{\Xk_{12}}{\Xk_{11}}e^{-\gamma_k(a_\sigma \Xk_{12}-(a_\sigma-2)\Xk_{11})}\\
  &=\frac{\sigma^2(n+1)}{\sigma^2(n+1)+2n}g_k e^{-\gamma_k(a_\sigma \Xk_{12}-(a_\sigma-2)\Xk_{11})}
\end{align*}
The induction hypothesis can be written as 
\begin{equation}\label{eq:inductionk}
a_\sigma \Xk_{12}-(a_\sigma-2)g_k\Xk_{11}=0,
\end{equation}
and combining \ref{lem:Xk_pop_dyn} with the fact that $\Xk\in \triangle_n$  we obtain
\begin{equation}\label{eq:X11X22}
    n\Xk_{11}+n(n-1)X_{12}.
\end{equation}
Using \eqref{eq:inductionk} and \eqref{eq:X11X22}, we deduce (by elementary calculations) that 
\[a_\sigma \Xk_{12}-(a_\sigma-2)\Xk_{11}=\frac{a_\sigma(a_\sigma-2)(g_k-1)}{a_\sigma+(a_\sigma-2)(n-1)g_k}.\]
Then for $\gamma_k$ chosen as 
\[\gamma_k=\frac{a_\sigma+(a_\sigma-2)(n-1)}{a_\sigma(a_\sigma-2)}\frac{g_k}{(g_k-1)}\log{\frac{g_k}{g_{k+1}}}\]
the property \eqref{eq:ratio_1211} is satisfied for $k+1$. 
\end{proof}
%Recalling the definition $a_\sigma:=2+\frac{n+1}n\sigma^2$, we use Lemma \ref{lem:sequence_gap_popdyn} to obtain that there exist a sequence $\{\gamma_k\}^\infty_{k=0}\in\matR_+$ such that $a_\sigma X^{(l)}_{12}-(a_\sigma-2)X^{(l)}_{11}>0$, for all $l\geq 1$. That, together with the following relation
%\begin{equation}\label{eq:X11X12}
%\frac{\Xk_{11}}{\Xk_{12}}= \frac{\Xzero_{11}}{\Xzero_{12}}\exp{\big(\sum^{k-1}_{l=0}\gamma_l(a_\sigma X^{(l)}_{12}-(a_\sigma-2) X^{(l)}_{11})\big)},
%\end{equation}
%will clearly imply the conclusion of the proposition. It only remains to verify the conditions of Lemma \ref{lem:sequence_gap_popdyn} are satisfied for some sequence $g_k$, which is equivalent to prove that the conditions $g_k>1$ for all $k\geq 1$ and $\frac{a_\sigma-2}{a_\sigma}g_k<1$ have non-empty intersection. But for this we can simply take any sequence $\{g_k\}^\infty_{k=1}\in(1,\frac{a_\sigma}{a\sigma-2})$, which exists because $\frac{a_\sigma}{a\sigma-2}>1$. The existence of the sequence $\{\gamma_k\}^\infty_{k=0}$ (and its specific form in function of $\{g_k\}^\infty_{k=0}$) it is guaranteed by Lemma \ref{lem:sequence_gap_popdyn}.

%remark prop.
\begin{remark}
Notice that the condition $\{g_k\}^\infty_{k=1}\in[1,\frac{a_\sigma}{a\sigma-2})$ in Lemma \ref{lem:sequence_gap_popdyn} becomes easier to be satisfied when $\sigma$ is small. In particular, for $\sigma=0$, we see that it is possible to take any sequence $\{g_k\}^\infty_{k=1}$, thus any sequence of strictly positive rates $\{\gamma_k\}^{\infty}_{k=0}$ will produce the desired outcome (diagonal dominance of $\Xk$ for all $k$). Notice that to obtain that to obtain that $\Xk_{11}>\Xk_{12}$ we need to prove a lower bound for $\Xk_{12}$ in terms of $\Xk_{11}$ (as it is clear from \eqref{eq:X11X12}).
\end{remark}

%remark prop partial fulfillment
%
\begin{remark}
 Lemma \ref{lem:sufficient_prop} gives a sufficient condition for the Algorithm \ref{alg:gmwm} to output $\id$, which involves the satisfaction of \eqref{eq:property} for all $i\neq j\in [n]$. A natural question is whether a partial fulfilment of \eqref{eq:property} can give perhaps a weaker conclusion, such as certain overlap with the $\id$ permutation. It is easy to see that this will depend not only on the number of pairs of indices that satisfy \eqref{eq:property}, but also on their respective location on the grid $[n]^2$. Indeed, take for example a matrix $C=J+\id+2D_{-1}$, where $D_{-1}$ is a matrix with $1$'s on the subdiagonal and $0$'s everywhere else. The matrix $C$, clearly satisfies the property \eqref{eq:property} for all $i,j$, except those in the subdiagonal, however $\texttt{GMWM}(C)$ has zero overlap with $\id$. On the other hand, if the set of indices that satisfy \eqref{eq:property} is of the form $\calI^2$ for $\calI\subset [n]$, and $|\calI|/n$ is large, then we $\texttt{GMWM}(C)$ will have non-trivial overlap with $\id$. If, for example, $|\calI|/n$ larger than $3/4$, then $\texttt{GMWM}(C)$ will have an overlap with the identity of at least $1/4$. 
\end{remark}%

%a family of discrete dynamics paragraph
\paragraph{A family of dynamics.} The mirror descent algorithm can be regarded as a family of discrete random dynamical systems, parametrized by a sequence of \emph{learning rates} $(\gamma_k)^\infty_{k=0}$. Similar to the gradient descent dynamics, the update on the state variable $\Xkone$ will depend on $\Xk$ and $\nabla E(\Xk;A,B
)$ (which is random because $A$ and $B$ are random). We can write the mirror descent dynamic for minimizing $E(\cdot)$ on $\simp$ in compact form, given a step size sequence $(\gamma_k)^\infty_{k=0}$, using entrywise exponentials, in the following way 
\begin{align}\label{eq:md_dynamic_init}
    \Xzero&=J/n,\\ \label{eq:md_dynamic_update}
    \Xkone&=n\cdot\frac{\Xk\odot e^{-\gamma_k\nabla E(\Xk)}}{\|\Xk\odot e^{-\gamma_k\nabla E(\Xk)}\|_{1,1}},
\end{align}
where $\nabla E(X;A,B)=A^2X+XB^2-2AXB$ (recalling the definition of $E(\cdot)$ in \eqref{def:obj_function}).
Notice that at iteration $k$, the candidate $X^{(k+1)}$ is obtained by an entrywise multiplication of the previous candidate, that is $X^{(k)}$, with the matrix $e^{-\gamma_k \nabla E(X^{k})}$, where we recall that, for $M\in\matR^{n\times n}$, $e^{M}$ represents the Hadamard (or entrywise) exponential, and then this entrywise product is normalized, using the $\|\cdot\|_{1,1}$ norm. 


%remark md n simplex
\begin{remark}[Derivation of mirror descent on the $n$-simplex]\label{rem:md_n_simplex}
For a given initial point $\tilde{X}^{(0)}\in \triangle_1$ and sequence of stepsizes $\{\tilde{\gamma}_k\}^{\infty}_{k=0}$, the mirror descent dynamics for optimizing $E(\cdot)$ on $\triangle_1$ are given by the update rule 
\begin{equation}\label{eq:md_unit_simplex}
    \tilde{X}^{(k+1)}=\frac{\tilde{X}^{(k)}\odot e^{-\tilde{\gamma}_k\nabla E(\tilde{X}^{(k)})}}{\|\tilde{X}^{(k)}\odot e^{-\tilde{\gamma}_k\nabla E(\tilde{X}^{(k)})}\|_{1,1}}.
\end{equation}
We consider the one-to-one map $\phi:\simp\rightarrow \triangle_1$, defined as $\phi(X)=\frac1nX$. Notice that $E(\phi(X))=\frac1{n^2}E(X)$, which implies that $X$ is a minimizer of $E(\cdot)$ on $\simp$ if and only if $\phi(X)$ is a minimizer of $E(\cdot)$ on $\triangle_1$. The mirror descent steps \eqref{eq:md_dynamic_init} and \eqref{eq:md_dynamic_update} are obtained as follows. At each step $k$, we first apply $\phi(\cdot)$ to $\Xk$, then use \eqref{eq:md_unit_simplex}, with $\tilde{X}^{(k)}=\phi(\Xk)$, to obtain $\tilde{X}^{(k+1)}$, and $\Xkone$ is simply defined as $\phi^{-1}(\tilde{X}^{(k+1)})$. Consequently, every trajectory $\{X^{(k)}\}^{\infty}_{k=0}$ of mirror descent on $\simp$ with step sizes $\gamma_k$ is one-to-one relation with a trajectory $\{\tilde{X}^{(k)}\}^{\infty}_{k=0}$ of mirror descent of $\triangle_1$, with $\tilde{X}^{(k)}=\phi(X^{(k)})$, and step sizes $\tilde{\gamma}_k=\frac1n\gamma_k$ (which is justified by the fact that $\nabla E(\cdot)$ is a linear function).
\end{remark}
%
%experiments properties etc 
\subsection{Experimental evidence for properties \ref{eq:property} and \ref{eq:property_sym} }
%
We present a series of experiments that show how the properties \eqref{eq:property} and \eqref{eq:property_sym}  evolve in average during the iterations of Algorithm \ref{alg:mirror_simplex}, and compare them with the diagonal dominance property and the overlap with the ground truth at each step. More specifically, we sample $A,B\sim\calW(n,\sigma,\Pi^*)$ for a random permutation $\Pi^*$ and consider $\Xk$ satisfying the dynamics defined by \eqref{eq:md_dynamic_init} and \eqref{eq:md_dynamic_update}, and for each $\Xk$ we compute four quantities: the percentage of pairs $(i,j)$ with $i\neq j$ that satisfy the \eqref{eq:property_sym}, the percentage of pairs $(i,j)$ with $i\neq j$ that satisfy the \eqref{eq:property}, the percentage of indices $i\in [n]$ such that the row $\Xk_{i:}$ is diagonally dominant and, lastly, the overlap between $\greedy(\Xk)$ and $\Pi^*$, which we call the percentage of recovery. Note that for this last quantity, we need to project onto the set of permutations, because we defined the overlap for a pair of permutations. Recall that, ultimately, is the percentage of recovery what measures the performance of the matching algorithms, then the idea is to see experimentally which, if any, of the sufficiency properties for perfect recovery given in Section \ref{sec:greedy} is more correlated with this performance measure.
%
In Fig. \ref{fig:prop.max}-\ref{fig:prop.sum} we show graphically the evolution of the following three properties, in terms of the iteration of Algorithm \ref{alg:mirror_simplex},
\begin{enumerate}[label=(\alph*)]
    \item \emph{Property max. }For a given time $k$, this is the fraction of pairs $(i,j)\in [n]^2$, with $i\neq j$, such that $\Xk_{ii}\vee \Xk_{jj}>\Xk_{ij}\vee\Xk_{ji}$. 
    \item \emph{Property sum. }For a given time $k$, we consider the number of $(i,j)\in [n]^2$, with $i\neq j$, such that $\Xk_{ii}+\Xk_{jj}>\Xk_{ij}+\Xk_{ji}$. 
    \item \emph{Property sum-max. }Similar to the previous definitions, but changing the condition to $\Xk_{ii}+\Xk_{jj}>\Xk_{ij}\vee\Xk_{ji}$.
\end{enumerate}
   %
    We used matrices generated with correlated Gaussian Wigner model, with $n=500,\sigma=1/20$, and set the parameter $N$ of Algorithm \ref{alg:mirror_simplex} to $36$. Each property is averaged over $25$ Monte Carlo runs. In addition, we track the recovery fraction after each iteration of Algorithm \ref{alg:mirror_simplex} and show its evolution in Fig. \ref{fig:recovery}. by looking at the shape of the curve, the property that seems more correlated with the recovery fraction is Property sum, but property sum-max seems very similar too. To tell them apart, we include an accompanying figure (generated using the same data) with the number of steps of the algorithm needed to reach its maximum possible value. Instead of averaging over the Monte Carlo runs, we show the situation at each Monte Carlo run. Here is clear that the Property max is the better correlated with the recovery. On the other hand, the Property sum-max reach its maximum level after the maximum level (it is sufficient, but no necessary) and the Property sum seems to not be sufficient. 
\begin{table}[h]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}\hline
    $k$ & $\sigma$ & $\%$ prop.sum & $\%$ prop.max & $\%$ diag.dom.&$\%$ recovery\\\hline \hline
    \multirow{3}{*}{1} & 0 & 100 &  100& 1.19&100\\ \cline{2-6}
    & 0.05 & 99.81 & 99.66&1.06&32.70\\\cline{2-6}
    & 0.1 & 99.32& 99.080&1.08&17.43\\ \hline
    \multirow{3}{*}{2} & 0 & 99.86 & 99.99&1.53&97.22\\ \cline{2-6}
    & 0.05 & 99.85 &99.79&1.27&46.99 \\\cline{2-6}
    & 0.1 & 99.73 &99.36& 1.53&27.62\\\hline
    \multirow{3}{*}{3} & 0 & 99.99 & 99.99& 2.20&99.97\\ \cline{2-6}
    & 0.05 & 99.99 &99.92& 1.96&72.61\\\cline{2-6}
    & 0.1 & 99.98 & 99.66&2.35&44.69\\\hline
    \multirow{3}{*}{4} & 0 & 99.99 & 99.99&3.15&99.98\\ \cline{2-6}
    & 0.05 & 99.99 &99.96& 2.93&88.10\\\cline{2-6}
    & 0.1 & 99.99 &99.80& 3.21&58.32\\\hline
    \multirow{3}{*}{5} & 0 & 100 & 100&3.98&100\\ \cline{2-6}
    & 0.05 & 99.99 &99.98& 3.61&93.44\\\cline{2-6}
    & 0.1 & 99.99 & 99.92&4.03&67.24\\\hline
    \multirow{3}{*}{6} & 0 & 100 & 100&4.68&100\\ \cline{2-6}
    & 0.05 & 100 &99.99& 4.29&96.66\\\cline{2-6}
    & 0.1 & 99.99 & 99.94&5.13&74.89\\\hline
    \multirow{3}{*}{7} & 0 & 100 & 100&5.14&100\\ \cline{2-6}
    & 0.05 & 100 &99.99& 4.90&98.23\\\cline{2-6}
    &0.1 & 99.99 &99.99& 5.42&81.15\\\hline
    \end{tabular}
    \caption{Summary of different statistics for sufficiency properties for ground truth recovery (see Lemma \ref{lem:sufficient_prop}). We show the average over $25$ Monte Carlo runs and the standard deviation on parenthesis. }
    \label{tab:properties_evol}
\end{table}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
            \centering\includegraphics[width=\textwidth]{images/prop_max.jpg}
            \caption[Property max]%
            {{\small Property max}}  \label{fig:prop.max}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
            \centering\includegraphics[width=\textwidth]{images/prop_sum_max.jpg}
            \caption[Property sum-max]%
            {{\small Property sum-max}}  \label{fig:prop.sum.max}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}
            \centering\includegraphics[width=\textwidth]{images/prop_sum.jpg}
            \caption[Property sum]%
            {{\small Property sum}}  \label{fig:prop.sum}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}
            \centering\includegraphics[width=\textwidth]{images/recovery.jpg}
            \caption[Recovery]%
            {{\small Recovery}}  \label{fig:recovery}
    \end{subfigure}
    \caption{Fraction of pairs that satisfy each property described in Section \ref{sec:greedy}. We consider $N=36$ in Algorithm \ref{alg:mirror_simplex} and average over $25$ Monte Carlo runs. Here $n=500$ and $\sigma=1/20$.}
    \label{fig:properties_fraction}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{images/iterations_bef_perfect.jpg}
    \caption{Number of iterations of Algorithm \ref{alg:mirror_simplex} that needed to be performed before each of the properties reach their maximum possible value. We used the same data that in Fig. \ref{fig:properties_fraction} ($n=500$,$\sigma=1/20$ and $N=36$).}\label{fig:iterations_before_perfect}
\end{figure}

%some text experiments
defined given the output of a convex relaxation for graph matching $\hat{X}$, the most common approach to prove $\greedy (\hat{X})=\id$, for a given similarity matrix is to prove that $\hat{X}$ satisfies the diagonal dominance property

==> previous_material/previous_setup.tex <==
%some od remarks....
\begin{remark}[Relation to anti-Monge matrices]
There is a relation between property \eqref{eq:property} and the set of \emph{strictly bottleneck anti-Monge} matrices \cite{BottleneckMonge,algebraicMonge}, which are the matrices $C\in\matR^{n\times n}$ that satisfy $C_{ij}\vee C_{kl}>C_{il}\vee C_{kj}$, for all $1\leq i<k\leq n$, $1\leq j<l\leq n$. Clearly, if a matrix belongs to the set of strictly bottleneck anti-Monge matrices, then it satisfy property \eqref{eq:property}. Similarly, a matrix belongs to the set of \emph{strict anti-Monge} matrices if $C_{ij}+ C_{kl}>C_{il}+ C_{kj}$, and if a matrix belongs to this set, then it also satisfy property \eqref{eq:property_sym}. The Monge property has been well studied in combinatorial optimization \cite{perspectiveMonge} and in several domains of applications. Recently, the problem of minimax estimation of Monge matrices was studied in \cite{estimationMonge}.
\end{remark}

\begin{remark}[Relation to diagonal dominance property]\label{rem:diag_dom}
A common strategy in the literature (see \cite{Grampa,ArayaBraunTyagi}) to prove that a GM algorithm succeeds (assuming that the ground truth is $\Pi^*=\id$) is to prove that a similarity matrix $C$ satisfy the following property, which is usually referred to as \emph{diagonal dominance}, $C_{ii}>C_{ij}$ for all $i\neq j$. Clearly, this diagonal dominance property implies \eqref{eq:property} (and \eqref{eq:property_sym} if $C$ is symmetric), thus it represents a stronger property. 

\end{remark}

%%Meta-algorithm
\subsection{A general algorithmic strategy}\label{sec:strategy}
The meta-strategy used by most graph matching algorithms (even those not directly based on convex relaxations) consists in two steps that can be summarized as follows,
\begin{enumerate}
    %
   \item \textbf{Similarity finding. } We find a data-dependent similarity matrix $\hat{X}$, whose $(i,j)-$th entry should capture, in informal terms, how likely is that $j$ is the image of $i$ under $\Pi^*$. When relying on a convex relaxation of graph matching, $\hat{X}$ will be precisely a solution of \eqref{eq:convex_relax_general}. In the case that $\calK$ is the set of matrices X that satisfy $\ones^TX\ones=n$, it has been shown in \cite{Grampa} that the solution has a closed-form expression in terms of the spectra of the pair of input graphs to be matched. However, for other choices of $\calK$ it is unclear that such a closed-form expression exists. 
   %
    \item \textbf{Rounding. } The similarity matrix $\hat{X}$, which typically contains entries in $\matR$, is rounded to matrix $\hat{X}_\calP$ with entries in $\{0,1\}$. This step can be accomplished by projecting $\hat{X}$ onto the set of permutations, which, when minimizing the Frobenius norm, is equivalent to solving a \emph{maximum linear assignment problem} with $\hat{X}$ playing the role of the cost matrix. Since analyzing linear assignment can be quite challenging, many algorithms opt for using a greedy rounding strategy. This approach is simpler to analyze, more computationally efficient, and in experimental results, it often exhibits comparable error rates to linear assignment.
    %
\end{enumerate}
%

